Fourier analysis of advection-dominated accretion flows

We implement a new semi-analytical approach to investigate radially self-similar solutions for the steady-state advection-dominated accretion flows (ADAFs). We employ the usual $\alpha$-prescription for the viscosity and all the components of the energy-momentum tensor are considered. In this case, in the spherical coordinate, the problem reduces to a set of eighth-order, nonlinear differential equations with respect to the latitudinal angle $\theta$. Using the Fourier expansions for all the flow quantities, we convert the governing differential equations to a large set of nonlinear algebraic equations for the Fourier coefficients. Using the Newton-Raphson method we solve the algebraic equations and ADAF properties are investigated over a wide range of the model parameters. We also show that the implemented series are truly convergent. The main advantage of our numerical method is that it does not suffer from the usual technical restrictions which may arise for solving ADAF differential equations near to the polar axis. In order to check the reliability of the approach, we recover some widely studied solutions. We also introduce a new varying $\alpha$ viscosity model and new outflow and inflow solutions for ADAFs are presented using Fourier expansion series.

==> Ref.tex <==

\begin{thebibliography}{}


\bibitem{} Anderson, L. D., Bania, T. M., Jackson, J. M., Clemens, D. P., Heyer, M., Simon, R., ... \& Rathborne, J. M., 2009, The Astrophysical Journal Supplement Series, 181, 1
\bibitem{} Binney, J. \& Tremaine, S., Galactic dynamics, 2011, Princeton university press
\bibitem{} Blandford R. \& Teukolsky S. A., 1969, Astrophys. J., 205, 55
\bibitem{} Boss, A. P., \& Sandra A. K. 2010, The Astrophysical Journal Letters, 717, L1
\bibitem{} Burke W. L.,1971, J. Math. Phys., 401
\bibitem{} Chandrasekhar, S. , 1967, Astrophys. J., 148, 621
\bibitem{} Chandrasekhar, S. \&  Nutku, Y., 1969, Astrophys. J., 158, 55
\bibitem{} Chandrasekhar, S. \& Esposito, F. P., 1970, Astrophys. J., 160, 153
\bibitem{} Chandrasekhar, S., 1965, Astrophys. J., 142, 1488
\bibitem{} Chandrasekhar, S.,1969 ,Astrophys. J., 158, 45
\bibitem{} Damour, T., \& Taylor, 1991, J. H., Astrophys. J., 366 , 501
\bibitem{} Demianski, M.\& Ivanov, P. B., 1997, Astronomy and Astrophysics, 324, 829
\bibitem{} Einstein, A., 1915, Preuss. Akad. Wiss. Berlin, 47, 831
\bibitem{} Epstein, R., 1977, Astrophys. J., 216, 92
\bibitem{} Faber, J. A., \& Rasio, F. A., 2000, Physical Review D, \textbf{62}, 6
\bibitem{} Guobin, M.,  et al., 2014,  The Astrophysical Journal, 790.2, 109
\bibitem{} Hulse, R. A. \& Taylor, J. H., 1975, Astrophys. J. Lett., 195, L51
\bibitem{} Kastner, J. H., et al., 2002, The Astrophysical Journal, 672.2, 957
\bibitem{} Kastner, J. H., Montez Jr, R., Balick, B., \& De Marco, O., 2008, The Astrophysical Journal, 672, 2
\bibitem{} Kimura, M., Tsunemi, H., Tomida, H., Sugizaki, M., Ueno, S., Hanayama, T., ... \& Sasaki, M. (2013). Publications of the Astronomical Society of Japan, 65(1), 14.
\bibitem{} Kohri, K., \&  Mineshige S., 2002, The Astrophysical Journal, 577.1, 311
\bibitem{} Lai, D., \& Wiseman, A. G., 1996, Physical Review D, 54, 6
\bibitem{} Latter, W. B., et al., 2000,  The Astrophysical Journal 539.2, 783
\bibitem{} Levenson, N. A., Graham, J. R., Aschenbach, B., Blair, W. P., Brinkmann, W., Busser, J. U., ... \& Klein, R. I. (1997), The Astrophysical Journal, 484(1)
\bibitem{} Masaru S., et al., 2006, Physical review letters, 96.3, 031102
\bibitem{} Masashi, K.,  et al., 2013, Publications of the Astronomical Society of Japan, 65.1, 14
\bibitem{} Masson, C. R. (1989). The Astrophysical Journal, 336
\bibitem{} Marcolino, W. L. F., Hillier, D. J., De Araujo, F. X., \& Pereira, C. B. (2007). The Astrophysical Journal, 654(2).
\bibitem{} Mo, H., Van den Bosch, F., White, S., 2010, Galaxy formation and evolution, Cambridge University Press 
\bibitem{} Mou, G., Yuan, F., Bu, D., Sun, M., \& Su, M. (2014). The Astrophysical Journal, 790(2), 109.
\bibitem{} Mufson, S. L., Lyon, J., \& Marionni, P. A. (1975). The Astrophysical Journal, 201
\bibitem{} Poisson, E. \& Will, C. M., 2014, Gravity: Newtonian, Post-Newtonian, Relativistic, Cambridge University Press
\bibitem{} Rezzolla, L. \& Zanotti O., Relativistic hydrodynamics, Oxford University Press
\bibitem{} Ruiz, N., et al., 2013, The Astrophysical Journal, 767.1, 35
\bibitem{} Will, C. M., in 300 Years of Gravitation, ed. S. Hawking and W. Israel, 1987, Cambridge, 80
\bibitem{} Will, C. M., in Proceedings of the Eighth Nishinomiya- Yukawa Memorial Symposium on Relativistic Cosmology, ed. M. Sasaki (Tokyo, 1994, Universal Academy Press)
\bibitem{} Will, C. M., 2011, PNAS, 108, 15
\bibitem{} Zhekov, S. A., \& M. Perinotto., 1996, Astronomy and Astrophysics, 309, 648

\bibitem{} Kim, W.-T., \& Ostriker, E. C. 2001, ApJ, 559, 70
\bibitem{} Toomre, A. 1964, ApJ, 139, 1217
\bibitem{} Vandervoort, P. O. 1970, ApJ, 161, 87
\bibitem{} Kato, S. 1972, PASJ, 24, 61
\bibitem{} Rafikov, R. R. 2001, MNRAS, 323, 445
\bibitem{} Romeo, A. B. 1992, MNRAS, 256, 307
\bibitem{} Romeo, A. B., \& Wiegert, J. 2011, MNRAS, 416, 1191
\bibitem{} Bertin, G., \& Romeo, A. B. 1988, A\&A, 195, 105
\bibitem{} Shadmehri M., Khajenabi F., 2012, MNRAS, 421, 841
\bibitem{} Jog, C. J., \& Solomon, P. M. 1984, ApJ, 276, 114
\bibitem{} Jog, C. J. 1996, MNRAS, 278, 209

\bibitem{} Elmegreen, B. G. 1987, ApJ, 312, 626
\bibitem{} Elmegreen, B. G. 1995, MNRAS, 275, 944
\bibitem{} Elmegreen, B. G. 2011, ApJ, 737, 1
\bibitem{} Gammie, C. F. 1996, ApJ, 462, 725
\bibitem{} 
  J.~Freundlich, C.~J.~Jog and F.~Combes,
  %``Local stability of a gravitating filament: a dispersion relation,''
  Astron.\ Astrophys.\  {\bf 564}, A7 (2014)
\bibitem{} 
  M.~Roshan and S.~Abbassi,
  %``Jeans analysis in modified gravity,''
  Phys.\ Rev.\ D {\bf 90}, no. 4, 044010 (2014)  
  \bibitem{}
  M.~Roshan and S.~Abbassi,
  %``On the stability of a galactic disk in modified gravity,''
  Astrophys.\ J.\  {\bf 802} (2015) no.1,  9
  \bibitem{} 
  M.~Roshan and S.~Abbassi,
  %``Local stability of self-gravitating disks in $f(R)$ gravity,''
  Astrophys.\ Space Sci.\  {\bf 358}, no. 1, 11 (2015)
  
  \bibitem{}
S.~Capozziello, M.~De Laurentis, I.~De Martino, M.~Formisano and S.D.~Odintsov, Phys.\ Rev. \ D {\bf 85}, 044022 (2012).

\bibitem{}
  L.~Blanchet,
  %``Gravitational radiation from post-Newtonian sources and inspiralling compact binaries,''
  Living Rev.\ Rel.\  {\bf 9} (2006) 4.
  \bibitem{} 
  C.~M.~Will,
  %``The Confrontation between general relativity and experiment,''
  Living Rev.\ Rel.\  {\bf 9}, 3 (2006)
  \bibitem{} 
  C.~J.~Jog,
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 434}, 56 (2013) 
  \bibitem{} 
  D.~M.~Siegel, R.~Ciolfi, A.~I.~Harte and L.~Rezzolla,
  Phys.\ Rev.\ D {\bf 87}, no. 12, 121302 (2013)
    \bibitem{} 
  Blandford R. D., Pringle J. E., 1976, MNRAS, 176, 443
    \bibitem{} 
  Ferrari A., Trussoni E., Zaninetti L., 1978, A\& A, 64, 43
  \bibitem{} 
  Zhang B., MacFadyen A., Wang P., 2009, ApJ, 692, L40
  \bibitem{} 
  Hardee P. E., Norman M. L., 1988, ApJ, 334, 70
\end{thebibliography}

==> aliases.tex <==
\usepackage{xspace}

%  FORMATS
\newcommand{\dspaceon}{\renewcommand{\baselinestretch}{1.1}\large\normalsize}
\newcommand{\dspaceoff}{\renewcommand{\baselinestretch}{1}\large\normalsize}
\newcommand{\footon}{\dspaceoff\footnotesize}
\newcommand{\bk}{\!\!\!\!}

% MATH
\newcommand{\mean}[1]{\ensuremath{\langle#1\rangle}}
\newcommand{\abs}[1]{\lvert#1\rvert} 
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\sub}[1]{\ensuremath{{_{\rm{#1}}}}}
\newcommand{\super}[1]{\ensuremath{{^{\rm{#1}}}}}
\newcommand{\rootn}{\ensuremath{\sqrt{n}}\xspace}

%  UNITS
\newcommand{\cps}{\,s$^{-1}$\xspace}
\newcommand{\un}[1]{\,\ensuremath{\rm{#1}}}
\newcommand{\as}{$^{\prime\prime}$\xspace}
\newcommand{\am}{$^{\prime}$\xspace}
\newcommand{\degrees}{$^{\circ}$}
\newcommand{\rsol}{\,$R_{\odot}$\xspace}
\newcommand{\lsol}{\,$L_{\odot}$\xspace}
\newcommand{\tsol}{\,$\tau_{\odot}$\xspace}
\newcommand{\msun}{\,$M_{\odot}$\xspace}
\newcommand{\msol}{\msun}
\newcommand{\lsun}{\,$L_{\odot}$\xspace}
\newcommand{\rsun}{\,$R_{\odot}$\xspace}
\newcommand{\msunperyear}{\msol\!$\rm yr^{-1}$\xspace}
\newcommand{\msolperyear}{\msunperyear}
\newcommand{\ergpersec}{\un{ergs\;s^{-1}}\xspace}
\newcommand{\ergpercmsec}{\un{ergs\,cm^{-2}\,s^{-1}}\xspace}
\newcommand{\percmsec}{\un{cm^{-2}\,s^{-1}}\xspace}
\newcommand{\percmsqrd}{\un{cm^{-2}}\xspace}
\newcommand{\phpercmseckev}{\un{ph\;cm^{-2}\,s^{-1}\,keV^{-1}}\xspace}
\newcommand{\phpercmsec}{\un{ph\;cm^{-2}\,s^{-1}}\xspace}
\newcommand{\rs}{\,$r_{\rm s}$\xspace}
\newcommand{\rlso}{\,$r_{\rm lso}$\xspace}
\newcommand{\rmso}{\,$r_{\rm mso}$\xspace}

%  INSTRUMENTS
\newcommand{\cgro}{{\em CGRO\/}\xspace}
\newcommand{\comptel}{{\small COMPTEL}\xspace}
\newcommand{\egret}{{\small EGRET}\xspace}
\newcommand{\integ}{{\sl INTEGRAL\/}\xspace}
\newcommand{\ibis}{{\small IBIS}\xspace}
\newcommand{\isgri}{{\small ISGRI}\xspace}
\newcommand{\picsit}{{\small PICSIT}\xspace}
\newcommand{\spi}{{\small SPI}\xspace}
\newcommand{\jemx}{{\small JEM-X}\xspace}
\newcommand{\omc}{{\small OMC}\xspace}
\newcommand{\hess}{{HESS}\xspace}

\newcommand{\fermi}{{\em Fermi}\xspace}
\newcommand{\uhuru}{{\em Uhuru}\xspace}
\newcommand{\ariel}{{\em Ariel\,V}\xspace}
\newcommand{\einstein}{{\em Einstein}\xspace}
\newcommand{\spacelab}{{\em Spacelab\,2}\xspace}
\newcommand{\xrt}{XRT\xspace}
\newcommand{\granat}{{\em Granat}\xspace}
\newcommand{\artp}{ART-P\xspace}
\newcommand{\sigm}{Sigma\xspace}
\newcommand{\ginga}{{\em Ginga}\xspace}
\newcommand{\asca}{{\em ASCA}\xspace}
\newcommand{\rosat}{{\em Rosat}\xspace}
\newcommand{\rxte}{{\small RXTE}\xspace}
\newcommand{\chandra}{{\em Chandra}\xspace}
\newcommand{\xmm}{{\em XMM-Newton}\xspace}
\newcommand{\suzaku}{{\em Suzaku}\xspace}
\newcommand{\epic}{{\small EPIC}\xspace}
\newcommand{\mos}{{\small MOS}\xspace}
\newcommand{\mosone}{{\small MOS1}\xspace}
\newcommand{\mostwo}{{\small MOS2}\xspace}
\newcommand{\pn}{{\small PN}\xspace}

\newcommand{\hst}{{\em HST\/}\xspace}
\newcommand{\hubble}{{\em Hubble Space Telescope\/}\xspace}
\newcommand{\keck}{{\it Keck}\xspace}
\newcommand{\cobe}{{\em COBE\/}\xspace}
\newcommand{\vla}{{\em VLA\/}\xspace}
\newcommand{\vlt}{{\em VLT\/}\xspace}


% SOURCES
\newcommand{\sgra}{Sgr\,A$^{*}$\xspace}
\newcommand{\sgraeast}{Sgr\,A\;East\xspace}
\newcommand{\sgrawest}{Sgr\;A\;West\xspace}
\newcommand{\igr}{IGR\,J17456--2901\xspace}
\newcommand{\ax}{AX\,J17456--2901\xspace}
\newcommand{\cxogc}{CXOGC\,J174540.0--290031\xspace}
\newcommand{\cxo}{\cxogc}
\newcommand{\xmmu}{XMMU\,J174554.4--285456\xspace}
\newcommand{\eg}{3EG\,J1746--2851\xspace}
\newcommand{\hessgc}{HESS\,J1745--290\xspace}


% WORDS
\newcommand{\afterTwoYears}{{\em A Persistent High-Energy Flux from the Heart of the Milky Way: INTEGRAL's View of the Galactic Center\/}\xspace}
\newcommand{\gammarays}{$\gamma$-rays\xspace}
\newcommand{\gammaray}{$\gamma$-ray\xspace}
\newcommand{\xray}{X-ray\xspace}
\newcommand{\xrays}{X-rays\xspace}
\newcommand{\fwhm}{FWHM\xspace}
\newcommand{\gti}{{\small GTI}\xspace}
\newcommand{\gtis}{{\small GTI}s\xspace}
\newcommand{\psla}{{\small PSLA}\xspace}
\newcommand{\arf}{{\small ARF}\xspace}
\newcommand{\arfs}{{\small ARF}s\xspace}
\newcommand{\rmf}{{\small RMF}\xspace}
\newcommand{\rmfs}{{\small RMF}s\xspace}
\newcommand{\pwn}{{\small PWN}\xspace}
\newcommand{\sn}{{\small SN}\xspace}
\newcommand{\snr}{{\small SNR}\xspace}
\newcommand{\snrs}{{\small SNR}s\xspace}
\newcommand{\gc}{{\small GC}\xspace}
\newcommand{\gcde}{{\small GCDE}\xspace}
\newcommand{\gd}{Galactic disk\xspace}
\newcommand{\gn}{{\small GN}\xspace}
\newcommand{\psf}{{\small PSF}\xspace}
\newcommand{\spsf}{{\small SPSF}\xspace}
\newcommand{\rms}{{\small RMS}\xspace}
\newcommand{\go}{{\small GO}\xspace}
\newcommand{\xspec}{{\small XSPEC}\xspace}
\newcommand{\glimpse}{{\small GLIMPSE}\xspace}
\newcommand{\ir}{{\small IR}\xspace}
\newcommand{\nir}{near-\ir}
\newcommand{\uv}{{\small UV}\xspace}
\newcommand{\ic}{{\small IC}\xspace}
\newcommand{\bh}{{\small BH}\xspace}
\newcommand{\osa}{{\small OSA}\xspace}
\newcommand{\sas}{{\small SAS}\xspace}
\newcommand{\isdc}{{\small ISDC}\xspace}
\newcommand{\ccd}{{\small CCD}\xspace}
\newcommand{\ccds}{{\small CCD}s\xspace}
\newcommand{\lmxb}{{\small LMXB}\xspace}
\newcommand{\lmxbs}{{\small LMXB}s\xspace}
\newcommand{\ism}{{\small ISM}\xspace}
\newcommand{\gmc}{{\small GMC}\xspace}
\newcommand{\gmcs}{{\small GMC}s\xspace}
\newcommand{\cmz}{{\small CMZ}\xspace}
\newcommand{\cnd}{{\small CND}\xspace}
\newcommand{\imf}{{\small IMF}\xspace}
\newcommand{\ura}{URA\xspace}
\newcommand{\mura}{MURA\xspace}
\newcommand{\og}{OG\xspace}
\newcommand{\ssc}{SSC\xspace}
\newcommand{\lso}{LSO\xspace}
\newcommand{\mso}{MSO\xspace}
\newcommand{\xrb}{XRB\xspace}
\newcommand{\xrbs}{XRBs\xspace}
\newcommand{\pdf}{{\small PDF\/}\xspace}
\newcommand{\cdf}{{\small CDF\/}\xspace}
\newcommand{\dof}{{\small DOF\/}\xspace}
\newcommand{\dft}{{\small DFT\/}\xspace}
\newcommand{\fft}{{\small FFT\/}\xspace}
\newcommand{\ifs}{{\small IFS\/}\xspace}
\newcommand{\psd}{{\small PSD\/}\xspace}
\newcommand{\pds}{{\small PDS\/}\xspace}


\newcommand{\hone}{H\,{\sc i\/}\xspace}
\newcommand{\htwo}{H\,{\sc ii\/}\xspace}
\newcommand{\neontwo}{Ne\,{\sc ii\/}\xspace}
\newcommand{\feone}{Fe\,{\sc i\/}\xspace}
\newcommand{\fetwentyfive}{Fe\,{\sc xxv\/}\xspace}
\newcommand{\fetwentysix}{Fe\,{\sc xxvi\/}\xspace}
\newcommand{\nione}{Ni\,{\sc i\/}\xspace}
\newcommand{\nitwentyseven}{Ni\,{\sc xxvii\/}\xspace}

